Patch Gradient Descent: Training Neural Networks on Very Large Images

Traditional CNN models are trained and tested on relatively low resolution images (<300 px), and cannot be directly operated on large-scale images due to compute and memory constraints. We propose Patch Gradient Descent (PatchGD), an effective learning strategy that allows to train the existing CNN architectures on large-scale images in an end-to-end manner. PatchGD is based on the hypothesis that instead of performing gradient-based updates on an entire image at once, it should be possible to achieve a good solution by performing model updates on only small parts of the image at a time, ensuring that the majority of it is covered over the course of iterations. PatchGD thus extensively enjoys better memory and compute efficiency when training models on large scale images. PatchGD is thoroughly evaluated on two datasets - PANDA and UltraMNIST with ResNet50 and MobileNetV2 models under different memory constraints. Our evaluation clearly shows that PatchGD is much more stable and efficient than the standard gradient-descent method in handling large images, and especially when the compute memory is limited.

==> tables/pandas-mbnet-1.tex <==
\begin{table}[]
\footnotesize
\centering
\begin{tabular}{@{}cccll@{}}
\toprule
Method & Resolution & Accuracy & QWK \\ \midrule
GD      & 512    &          &     \\
GD-extended      & 512               &          &     \\
PatchGD       & 512       &          &     \\
GD      & 1024    &          &     \\
GD-extended      & 1024               &          &     \\
PatchGD       & 1024       &          &     \\
GD      & 2048    &          &     \\
GD-extended      & 2048               &          &     \\
PatchGD       & 2048       &          &     \\
\bottomrule
\end{tabular}
\caption{Performance scores for standard Gradient Descent and our PatchGD method on the task of PANDAS classification using MobilenetV2 
architecture.}
\label{tab:sampling_ablation}
\end{table}
